Vehicle Routing Problems in the Age of Semi-Autonomous Driving

We are in the midst of a semi-autonomous era in urban transportation in which varying forms of vehicle autonomy are gradually being introduced. This phase of partial autonomy is anticipated by some to span a few decades due to various challenges, including budgetary constraints to upgrade the infrastructure and technological obstacles in the deployment of fully autonomous vehicles (AV) at scale. In this study, we introduce the vehicle routing problem in a semi-autonomous environment (VRP-SA) where the road network is not fully AV-enabled in the sense that a portion of it is either not suitable for AVs or requires additional resources in real-time (e.g., remote control) for AVs to pass through. Moreover, such resources are scarce and usually subject to a budget constraint. An exact mixed-integer linear program (MILP) is formulated to minimize the total routing cost of service in this environment. We propose a two-phase algorithm based on a family of feasibility recovering sub-problems (FRP) to solve the VRP-SA efficiently. Our algorithm is implemented and tested on a new set of instances that are tailored for the VRP-SA by adding stratified grid road networks to the benchmark instances. The result demonstrates a reduction of up to 37.5% in vehicle routing costs if the fleet actively exploits the AV-enabled roads in the environment. Additional analysis reveals that cost reduction is higher with more budget and longer operational hours.

==> figures/expanded_graph.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \begin{tikzpicture}

    % Vertex style
    % \SetVertexStyle{LineWidth = 2pt}
    
    % Based layer
    \Vertex[x = -2.8, y = -2.5, size = 0.01, style = {color = vertexfill}]{s}
    
    \Vertex[x = 0, y = -2, size = 0.01, style = {color = Orchid}]{1-0}
    \Vertex[x = 2.5, y = -1.5, size = 0.01, style = {color = Orchid}]{1-1}
    \Vertex[x = -1.25, y = -1.5, size = 0.01, color = black]{1-2}
    \Vertex[x = -2.5, y = -2.5, size = 0.01, style = {color = vertexfill}]{1-3}
    \Vertex[x = 1.25, y = -2.5, size = 0.01, color = black]{1-4}

    \Edge[lw = 0.5pt](1-1)(1-2)
    \Edge[lw = 0.5pt](1-2)(1-3)
    \Edge[lw = 0.5pt](1-3)(1-4)
    \Edge[lw = 0.5pt](1-1)(1-4)
    

    \Edge[lw = 0.5pt](1-0)(1-1)
    \Edge[lw = 0.5pt](1-2)(1-0)
    \Edge[lw = 0.5pt](1-3)(1-0)
    \Edge[lw = 0.5pt](1-4)(1-0)
    


    % Middle layer
    \Vertex[x = 0, y = 0, size = 0.01, style = {color = Orchid}]{2-0}
    \Vertex[x = 2.5, y = 0.5, size = 0.01, style = {color = Orchid}]{2-1}
    \Vertex[x = -1.25, y = 0.5, size = 0.01, color = black]{2-2}
    \Vertex[x = -2.5, y = -0.5, size = 0.01, style = {color = vertexfill}]{2-3}
    \Vertex[x = 1.25, y = -0.5, size = 0.01, color = black]{2-4}

    \Edge[lw = 0.5pt, style={dashed}](2-1)(2-2)
    \Edge[lw = 0.5pt, style={dashed}](2-2)(2-3)
    \Edge[lw = 0.5pt, style={dashed}](2-3)(2-4)
    \Edge[lw = 0.5pt, style={dashed}](2-1)(2-4)
    \Edge[style={dashed}, lw = 0.5pt](2-0)(2-1)
    \Edge[lw = 0.5pt, style={dashed}](2-0)(2-2)
    \Edge[lw = 0.5pt, style={dashed}](2-0)(2-3)
    \Edge[lw = 0.5pt, style={dashed}](2-0)(2-4)


    % Upper layer
    \Vertex[x = 0, y = 2, size = 0.01, style = {color = Orchid}]{3-0}
    \Vertex[x = 2.5, y = 2.5, size = 0.01, style = {color = Orchid}]{3-1}
    \Vertex[x = -1.25, y = 2.5, size = 0.01, color = black]{3-2}
    \Vertex[x = -2.5, y = 1.5, size = 0.01, style = {color = vertexfill}]{3-3}
    \Vertex[x = 1.25, y = 1.5, size = 0.01, color = black]{3-4}

    \Edge[lw = 0.5pt, style={dashed}](3-1)(3-2)
    \Edge[lw = 0.5pt, style={dashed}](3-2)(3-3)
    \Edge[lw = 0.5pt, style={dashed}](3-3)(3-4)
    \Edge[lw = 0.5pt, style={dashed}](3-1)(3-4)

    \Edge[style={dashed}, lw = 0.5pt](3-1)(3-0)
    \Edge[lw = 0.5pt, style={dashed}](3-2)(3-0)
    \Edge[style={dashed}, lw = 0.5pt](3-0)(3-3)
    \Edge[lw = 0.5pt, style={dashed}](3-4)(3-0)
    


    % Artificial edges
    \Edge[style={dashed}, lw = 2pt, Direct](1-0)(2-0)
    \Edge[style={dashed}, lw = 2pt, Direct](2-0)(3-0)
    \Edge[style={dashed}, lw = 2pt, Direct](1-1)(2-1)
    \Edge[style={dashed}, lw = 2pt, Direct](2-1)(3-1)

    \Edge[style={dashed}, Direct, bend = -45, lw = 2pt](2-3)(s)
    \Edge[style={dashed}, Direct, bend = -45, lw = 2pt](3-3)(s)

    
    \end{tikzpicture}
    \caption{A 3-Layer expanded graph of a tiny undirected road network}
    \label{fig:expanded_graph}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \begin{tikzpicture}

    % Vertex style
    % \SetVertexStyle{LineWidth = 2pt}
    
    % Based layer
    \Vertex[x = -2.8, y = -2.5, size = 0.01, style = {color = vertexfill}]{s}
        
    \Vertex[x = 0, y = -2, size = 0.01, style = {color = Orchid}]{1-0}
    \Vertex[x = 2.5, y = -1.5, size = 0.01, style = {color = Orchid}]{1-1}
    \Vertex[x = -1.25, y = -1.5, size = 0.01, color = black]{1-2}
    \Vertex[x = -2.5, y = -2.5, size = 0.01, style = {color = vertexfill}]{1-3}
    \Vertex[x = 1.25, y = -2.5, size = 0.01, color = black]{1-4}

    \Edge[lw = 0.5pt](1-1)(1-2)
    \Edge[lw = 0.5pt](1-2)(1-3)
    \Edge[lw = 0.5pt](1-3)(1-4)
    \Edge[lw = 0.5pt](1-1)(1-4)
    

    \Edge[lw = 0.5pt](1-0)(1-1)
    \Edge[lw = 0.5pt](1-2)(1-0)
    \Edge[color = red, lw = 2pt, Direct](1-3)(1-0)
    \Edge[lw = 0.5pt](1-4)(1-0)
    


    % Middle layer
    \Vertex[x = 0, y = 0, size = 0.01, style = {color = Orchid}]{2-0}
    \Vertex[x = 2.5, y = 0.5, size = 0.01, style = {color = Orchid}]{2-1}
    \Vertex[x = -1.25, y = 0.5, size = 0.01, color = black]{2-2}
    \Vertex[x = -2.5, y = -0.5, size = 0.01, style = {color = vertexfill}]{2-3}
    \Vertex[x = 1.25, y = -0.5, size = 0.01, color = black]{2-4}

    \Edge[lw = 0.5pt, style = {dashed}](2-1)(2-2)
    \Edge[lw = 0.5pt, style = {dashed}](2-2)(2-3)
    \Edge[lw = 0.5pt, style = {dashed}](2-3)(2-4)
    \Edge[lw = 0.5pt, style = {dashed}](2-1)(2-4)
    \Edge[color = red, style={dashed}, lw = 2pt, Direct](2-0)(2-1)
    \Edge[lw = 0.5pt, style = {dashed}](2-0)(2-2)
    \Edge[lw = 0.5pt, style = {dashed}](2-0)(2-3)
    \Edge[lw = 0.5pt, style = {dashed}](2-0)(2-4)
    

    % Upper layer
    \Vertex[x = 0, y = 2, size = 0.01, style = {color = Orchid}]{3-0}
    \Vertex[x = 2.5, y = 2.5, size = 0.01, style = {color = Orchid}]{3-1}
    \Vertex[x = -1.25, y = 2.5, size = 0.01, color = black]{3-2}
    \Vertex[x = -2.5, y = 1.5, size = 0.01, style = {color = vertexfill}]{3-3}
    \Vertex[x = 1.25, y = 1.5, size = 0.01, color = black]{3-4}

    \Edge[lw = 0.5pt, style = {dashed}](3-1)(3-2)
    \Edge[lw = 0.5pt, style = {dashed}](3-2)(3-3)
    \Edge[lw = 0.5pt, style = {dashed}](3-3)(3-4)
    \Edge[lw = 0.5pt, style = {dashed}](3-1)(3-4)

    \Edge[color = red, style={dashed}, lw = 2pt, Direct](3-1)(3-0)
    \Edge[lw = 0.5pt, style = {dashed}](3-2)(3-0)
    \Edge[color = red, style={dashed}, lw = 2pt, Direct](3-0)(3-3)
    \Edge[lw = 0.5pt, style = {dashed}](3-4)(3-0)
    

    % Artificial edges
    \Edge[color = red, style={dashed}, lw = 2pt, Direct](1-0)(2-0)
    \Edge[style={dashed}, lw = 2pt, Direct](2-0)(3-0)
    \Edge[style={dashed}, lw = 2pt, Direct](1-1)(2-1)
    \Edge[color = red, style={dashed}, lw = 2pt, Direct](2-1)(3-1)

    \Edge[style={dashed}, Direct, bend = -45, lw = 2pt](2-3)(s)
    \Edge[color = red, style={dashed}, Direct, bend = -45, lw = 2pt](3-3)(s)
    
    \end{tikzpicture}
    \caption{An optimal route in the expanded graph in Figure \ref{fig:expanded_graph}}
    \label{fig:optimal_route}
    \end{subfigure}

\caption{Illustration of a $3$-layer expanded graph}
\end{figure}
